Multi-Agent Inverse Reinforcement Learning in Real World Unstructured Pedestrian Crowds

Social robot navigation in crowded public spaces such as university campuses, restaurants, grocery stores, and hospitals, is an increasingly important area of research. One of the core strategies for achieving this goal is to understand humans' intent--underlying psychological factors that govern their motion--by learning their reward functions, typically via inverse reinforcement learning (IRL). Despite significant progress in IRL, learning reward functions of multiple agents simultaneously in dense unstructured pedestrian crowds has remained intractable due to the nature of the tightly coupled social interactions that occur in these scenarios \textit{e.g.} passing, intersections, swerving, weaving, etc. In this paper, we present a new multi-agent maximum entropy inverse reinforcement learning algorithm for real world unstructured pedestrian crowds. Key to our approach is a simple, but effective, mathematical trick which we name the so-called tractability-rationality trade-off trick that achieves tractability at the cost of a slight reduction in accuracy. We compare our approach to the classical single-agent MaxEnt IRL as well as state-of-the-art trajectory prediction methods on several datasets including the ETH, UCY, SCAND, JRDB, and a new dataset, called Speedway, collected at a busy intersection on a University campus focusing on dense, complex agent interactions. Our key findings show that, on the dense Speedway dataset, our approach ranks 1st among top 7 baselines with >2X improvement over single-agent IRL, and is competitive with state-of-the-art large transformer-based encoder-decoder models on sparser datasets such as ETH/UCY (ranks 3rd among top 7 baselines).

==> images/BCvsMAIRL.tex <==
\begin{figure}[t]
\centering
   \begin{subfigure}[h]{.49\columnwidth}
    \includegraphics[width=\textwidth]{images/simulation/mairl.png}
    \caption{Multi agent IRL~\cite{mairl}}
    \label{fig: mairl_vs_bc1}
  \end{subfigure}
  %
 \begin{subfigure}[h]{.49\columnwidth}
    \includegraphics[width=\textwidth]{images/simulation/BC.png}
    % \includegraphics[width=\textwidth]{images/mairl/rld.png}
    \caption{Behavior cloning~\cite{BC-transformer}}
    \label{fig: mairl_vs_bc2}
  \end{subfigure}
\caption{\textbf{Simulation and Partial conditioning:} We show that IL algorithms succeed when provided global information either in simulation \textit{(left)} or via partial conditioning \textit{(right)}.} 
  \label{fig: mairl_vs_bc}
  % \vspace{-15pt}
\end{figure}  


==> images/main_results_2.tex <==
\begin{figure}[t]
\centering
   \begin{subfigure}[h]{0.485\columnwidth}
    \includegraphics[width=\textwidth]{images/new_baselines/rld_implicit.png}
    \caption{Implicit BC~\cite{florence2022implicit}}
    \label{fig: ibc}
  \end{subfigure}
  %
  %  \begin{subfigure}[h]{0.24\textwidth}
  %   \includegraphics[width=\textwidth]{images/new_baselines/rld_gmm_mlp.png}
  %   \caption{GMM-MLP}
  %   \label{fig: gmmmlp}
  % \end{subfigure}
  % %
  %  \begin{subfigure}[h]{0.24\textwidth}
  %   \includegraphics[width=\textwidth]{images/new_baselines/rld_gmm_lstm.png}
  %   \caption{GMM-LSTM}
  %   \label{fig: gmmlstm}
  % \end{subfigure}
  %
     \begin{subfigure}[h]{0.485\columnwidth}
    \includegraphics[width=\textwidth]{images/new_baselines/rld_gmm_transformer.png}
    \caption{GMM}
    \label{fig: gmmtransformer}
  \end{subfigure}
\caption{Two additional baselines.} 
  \label{fig: main_results_2}
  \vspace{-10pt}
\end{figure}  

==> images/overview.tex <==
\begin{figure*}[t]
\centering
   \begin{subfigure}[h]{.32\textwidth}
    \includegraphics[width=\textwidth]{images/cover.png}
    \caption{}
    \label{fig: overview1}
  \end{subfigure}
  %
 \begin{subfigure}[h]{.32\textwidth}
    \includegraphics[width=\textwidth]{images/cover.png}
    \caption{}
    \label{fig: overview1}
  \end{subfigure}
    %
 \begin{subfigure}[h]{.32\textwidth}
    \includegraphics[width=\textwidth]{images/cover.png}
    \caption{}
    \label{fig: overview3}
  \end{subfigure}
\caption{\textbf{Speedway Dataset}--We depict representative images from the Speedway dataset comprising of pedestrian crowds, collected at the Speedway and $24^\textrm{th}$ intersection on the University of Texas at Austin campus. \rohan{will be replaced} } 
  \label{fig: overview}
  % \vspace{-10pt}
\end{figure*}  


==> tables/BC.tex <==
\begin{table}[t]
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
Method & Number of trajectories & \multicolumn{4}{c}{RMSE}\\
&&$16$s&$32$s&$48$s&$64$s\\
      \midrule
BC&$2000$&&&&\\
         \bottomrule
    \end{tabular}
    % }
    \caption{Evaluation Results}
    \label{tab: BC}
\end{table}

==> tables/dataset_comparison.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{rcccc}
    \toprule
    Dataset & \multicolumn{4}{c}{Description}\\
    \midrule
    &Structured& Unstructured & \makecell{Agents \\ involved} & \makecell{Density \\(\# agents / sq. meter)}\\
    \cmidrule{2-5}
       ETH/UCY~\cite{pellegrini2010eth}  & \cellcolor{red!25}\xmark& \cellcolor{red!25}\xmark & \cellcolor{red!25}- & \cellcolor{red!25}- \\
       SCAND~\cite{scand}  & \cellcolor{red!25}\xmark& \cellcolor{red!25}\xmark & \cellcolor{red!25}- & \cellcolor{red!25}- \\
       JRDB~\cite{jrdb} & \cellcolor{red!25}\xmark& \cellcolor{red!25}\xmark &\cellcolor{red!25} -& \cellcolor{red!25}-\\
       Waymo~\cite{waymo}  &\cmark (0.336 bits) & \cellcolor{red!25}\xmark & \cellcolor{red!25}Vehicles & \cellcolor{red!25}$1$\\
      INTERACTION~\cite{zhan2019interaction}  &\cmark (0.475 bits)& \cellcolor{red!25}\xmark & \cellcolor{red!25}Vehicles & \cellcolor{red!25}$1$\\
       \midrule
       \textbf{Speedway} &\xmark&\cellcolor{green!25}\cmark (1.061 bits)&\cellcolor{green!25}\textbf{Pedestrians and Vehicles} & \cellcolor{green!25}$\mathbf{3-4}$\\ 
       \bottomrule
    \end{tabular}}
    \caption{Comparing the Speedway dataset with  state-of-the-art trajectory planning datasets: Our dataset features trajectories of pedestrians as well as vehicles characterized by higher entropy (greater unpredictability) and increased density.}
    \label{tab: data_comparison}
    % \vspace{-15pt}
\end{table}

==> tables/methods.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{cc}
    \multicolumn{2}{c}{Methods}\\
       Inverse Reinforcement Learning  & Behavior Cloning \\
        MaxEnt IRL & \\ 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
